The Deep Latent Space Particle Filter for Real-Time Data Assimilation with Uncertainty Quantification

In Data Assimilation, observations are fused with simulations to obtain an accurate estimate of the state and parameters for a given physical system. Combining data with a model, however, while accurately estimating uncertainty, is computationally expensive and infeasible to run in real-time for complex systems. Here, we present a novel particle filter methodology, the Deep Latent Space Particle filter or D-LSPF, that uses neural network-based surrogate models to overcome this computational challenge. The D-LSPF enables filtering in the low-dimensional latent space obtained using Wasserstein AEs with modified vision transformer layers for dimensionality reduction and transformers for parameterized latent space time stepping. As we demonstrate on three test cases, including leak localization in multi-phase pipe flow and seabed identification for fully nonlinear water waves, the D-LSPF runs orders of magnitude faster than a high-fidelity particle filter and 3-5 times faster than alternative methods while being up to an order of magnitude more accurate. The D-LSPF thus enables real-time data assimilation with uncertainty quantification for physical systems.

==> old_text.tex <==
\section{Particle Filter} \label{section:sequential_monte_carlo}
PF methods are family of Monte Carlo methods that sample from a sequence of target (posterior) distributions. This section is partially based on \cite{wu2017sequential}.

The general idea behind all PF methods is to approximate the posterior pdf by a set of particles (samples) and corresponding weights:
\begin{align} \label{eq:discrete_posterior}
    p^{N}(\boldsymbol{u}_{n+1}| \boldsymbol{y}_{0:n+1}) = \sum_{i=1}^N w_{n+1}^{i} \delta\left(\boldsymbol{u}_{n+1} - \boldsymbol{u}_{n+1}^{i}\right),
\end{align}
where $\boldsymbol{u}_{n+1}^{i}$ is particle $i$ at time step $n+1$ and $w_{n+1}^{i}$ is it's corresponding weight. $p^{N}$ is referred to as the empirical density made up of $N$ particles. Various versions of PF methods differentiates in how the weights are computed. 
\begin{comment}
For the family of PF methods referred to as Sequential Importance Sampling (SIS), the weights are updated by:
\begin{align}
    \tilde{w}_{n+1}^{(i)} = \tilde{w}(\boldsymbol{u}_{n+1}) = w(\boldsymbol{u}_{n}) \frac{p(\boldsymbol{u}_{n+1} | \boldsymbol{u}_{n})p(\boldsymbol{y}_{n+1}|\boldsymbol{u}_{n+1})}{q(\boldsymbol{u}_{n+1}|\boldsymbol{u}_{n}, \boldsymbol{y}_{n+1})},
\end{align}
where $w$ is the importance weight function and $q$ is the proposal distribution. The choice of proposal distribution is a crucial choice and is subject to much research. We will come back to this in the next subsection.

\begin{align}
    q(\boldsymbol{u}_{n+1}|\boldsymbol{u}_{n}, \boldsymbol{y}_{n+1}) = p(\boldsymbol{u}_{n+1} | \boldsymbol{u}_{n}),
\end{align}
\end{comment}

Generally, there are three steps to a PF algorithm:
\begin{enumerate}
    \item Sampling;
    \item Weight update;
    \item Resampling.
\end{enumerate}
These are visualized in Figure \ref{fig:smc_procedure}. The \textit{sampling} step involves sampling from the transition distribution. Hence, it requires time stepping using the forward map $N$ times. The \textit{weight update} step involves updating the weights based on the chosen algortihm. Lastly, in the \textit{resampling} step, we resample the particles based on the weights. We do not resample at every time step, but only when the effective sample size (ESS),
\begin{align}
    ESS = \frac{N}{\sum_{j=1}^N \left(w_{n+1}^{j}\right)^2},
\end{align}
is small enough. Intuitively, the ESS indicates how diverse the ensemble of particles is.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/smc_procedure.png}
    \caption{Temporary figure!!!}
    \label{fig:smc_procedure}
\end{figure}

\subsection{Bootstrap Filter}
The bootstrap filter is a specific case of a sequential importance sampling PF. It is defined by choosing the proposal density to be the transition density, which gives the weight update:
\begin{align}
w_{n+1}^{i} = w(\boldsymbol{u}_{n}^{i})\frac{p(\boldsymbol{y}_{n+1}|\boldsymbol{u}_{n+1}^{i})}{\sum_{j=1}^N p(\boldsymbol{y}_{n+1}|\boldsymbol{u}_{n+1}^{j})}. 
\end{align}
Hence, in the bootstrap filter we update the weights only based on the likelihood. This makes it a very popular choice due to its simplicity.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/bootstrap_filter.png}
    \caption{Temporary figure!!!}
    \label{fig:smc_procedure}
\end{figure}

While being relatively simple, the bootstrap filter is typically computationally quite heavy. When the augmented state space and/or the observation space is high-dimensional it is necessary to compute many particles to get a good approximation of the true densities. Furthermore, for complex cases it is computationally intensive to sample from the transition distribution as we need to time step using the discretized PDE, $F$, for each particle. Therefore, it is infeasible to run the bootstrap filter in real-time for high-dimensional and/or nonlinear PDEs. We specifically aim to alleviate this by replacing the computational bottlenecks with deep learning-based surrogate models. 



\section{Neural Network Surrogate Model} \label{section:neural_networks}

As mentioned above, particle filters are rarely feasible to run in real-time due to the necessity of large ensembles and expensive PDEs. By speeding up the forward model, this can be alleviated. We aim to this by making use of neural network-based surrogate models.

In this section we present the two types of neural network frameworks: Wasserstein autoencoders and transformers. Autoencoders learn a low-dimensional representation of data and transformers learn to time-step in the low-dimensional space. 

\subsection{Autoencoders}
Autoencoders (AEs) are a type of neural networks that aims to identify a low-dimensional representation of data. The low-dimensional representation is referred to as the latent state. 
AEs consist of two neural networks: An encoder, $\phi_{\text{enc}}$, that reduces the dimension of the data, and a decoder, $\phi_{\text{dec}}$, that reconstructs the data. That is, 
\begin{align}
    \phi_{\text{enc}}(\boldsymbol{q}) = \boldsymbol{z}, \quad \phi_{\text{dec}}(\boldsymbol{z}) = \tilde{\boldsymbol{q}}, \quad \phi_{\text{dec}}(\phi_{\text{enc}}(\boldsymbol{q})) = \tilde{\boldsymbol{q}} \approx \boldsymbol{q}. 
\end{align}
AEs are trained by minimizing the mean squared error (MSE) between the input and the reconstruction. Hence, for a given training set, $\left\{\boldsymbol{q}_i\right\}_{i=0}^{N_{\text{train}}}$, the loss function is given by:
\begin{align}
    L(\phi_{\text{enc}}, \phi_{\text{dec}}) = \frac{1}{N_{\text{train}}} \sum_{i=1}^{N_{\text{train}}} \left(\boldsymbol{q}_i - \phi_{\text{dec}}(\phi_{\text{enc}}(\boldsymbol{q}_i)) \right)^2.
\end{align}
$L$ is minimized with respect to the weights of $\phi_{\text{enc}}$ and $\phi_{\text{dec}}$ typically using stochastic gradient descent type algorithms. Note that an $L^2$ or $L^1$ regularization term, regularization the weights of the neural networks, is often added to ensure generalization. In Figure \ref{fig:conv_AE} an illustration of an AE using convolutional neural networks is shown. 

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/conv_AE.eps}
    \caption{Illustration of a convlolutional AE. WILL BE UPDATED LATER!!!}
    \label{fig:conv_AE}
\end{figure}

\subsubsection{Wasserstein Autoencoders}
While AEs provide a  framework for computing latent representations of data, they lack certain properties that are of interest when computations in the latent space are necessary. Specifically, small perturbations in the latent space should result in small perturbations in the high-fidelity space as well. Moreover, it should be possible to sample from the latent space. By using so-called Wasserstein AEs (WAEs) \cite{tolstikhin2017wasserstein}, we can obtain these properties.

We introduce a prior distribution on the latent space, $P(\boldsymbol{z})$. While the encoder and decoder remain deterministic mappings, they define the conditional distributions $P_{\text{enc}}(\boldsymbol{z} | \boldsymbol{q})$ and $P_{\text{dec}}(\boldsymbol{q} | \boldsymbol{z})$, respectively, by the density functions:
\begin{align}
    p(\boldsymbol{z}) 
    &= 
    \int p(\boldsymbol{z} | \boldsymbol{q}) p(\boldsymbol{q}) \text{d}\boldsymbol{q} 
    \approx 
    \int p_{\text{enc}}(\boldsymbol{z} | \boldsymbol{q}) p(\boldsymbol{q}) \text{d}\boldsymbol{q} 
    =
    p_{\text{enc}}(\boldsymbol{z}),
    \\
    p(\boldsymbol{q}) 
    &= \int p(\boldsymbol{q} | \boldsymbol{z}) p(\boldsymbol{z}) \text{d}\boldsymbol{z} 
    \approx 
    \int p_{\text{dec}}(\boldsymbol{q} | \boldsymbol{z}) p(\boldsymbol{z}) \text{d}\boldsymbol{z} 
    =
    p_{\text{dec}}(\boldsymbol{q}),
\end{align}
The goal is to ensure that the encoder approximates the latent prior distribution, $p(\boldsymbol{z})\approx p_{\text{enc}}(\boldsymbol{z})$ and the decoder approximates the high-fidelity prior distribution, $p(\boldsymbol{q})\approx p_{\text{dec}}(\boldsymbol{q})$. This is achieved by simultaneously minimizing the reconstruction error and a divergence, $D$, between $p(\boldsymbol{z})$ and  $p_{\text{enc}}(\boldsymbol{z})$ that measures the similarity of the two distributions:
\begin{align}
    L_{\text{WAE}}(\phi_{\text{enc}}, \phi_{\text{dec}}) 
    = 
    \underbrace{
    \frac{1}{N} \sum_{i=1}^{N} \left(\boldsymbol{q}_i - \phi_{\text{dec}}(\phi_{\text{enc}}(\boldsymbol{q}_i)) \right)^2
    }_{\text{reconstruction}}
    +
    \lambda 
    \underbrace{D(p(\boldsymbol{z}), p_{\text{enc}}(\boldsymbol{z}))}_{\text{divergence}} 
    + 
    \alpha \underbrace{R(\phi_{\text{enc}}, \phi_{\text{dec}})}_{\text{regularization}}.
\end{align}
Here, $\lambda$ is another regularization parameter to be determined through hyperparameter tuning. In this paper, we choose the maximum mean discrepancy (MMD) with a multiquadratics kernel for the divergence, which gives us the WAE-MMD. In \cite{tolstikhin2017wasserstein}, it was argued that this is a good choice when $p(\boldsymbol{z})$ is normally distributed. Summarizing, by choosing the squared error cost function, together with the MMD divergence, we find:
\begin{align}
    L_{\text{WAE}}(\phi_{\text{enc}}, \phi_{\text{dec}}) 
    &= 
    \frac{1}{N} \sum_{i=1}^{N} \left(\boldsymbol{q}_i - \phi_{\text{dec}}(\phi_{\text{enc}}(\boldsymbol{q}_i)) \right)^2
     + \lambda \text{MMD}\left(\phi_{\text{enc}}, \left\{\boldsymbol{z}_i\right\}_{i=1}^{N} \right)
    + 
    \alpha R(\phi_{\text{enc}}, \phi_{\text{dec}}), \quad \boldsymbol{z}_i\sim P(\boldsymbol{z}).
\end{align}
where
\begin{align}
    \text{MMD}\left(\phi_{\text{enc}}, \left\{\boldsymbol{z}_i\right\}_{i=1}^{N} \right)
    =
    \frac{\lambda }{N(N-1)} \sum_{l\neq j}^{N}
    \left[k(\boldsymbol{z}_l, \boldsymbol{z}_j) + k(\phi_{\text{enc}}(\boldsymbol{q}_l), \phi_{\text{enc}}(\boldsymbol{q}_j))\right]
    + 
    \frac{2\lambda }{N^2} \sum_{l, j}^{N} k(\boldsymbol{z}_l, \phi_{\text{enc}}(\boldsymbol{q}_j),
\end{align}
and
\begin{align}
    k(\boldsymbol{z}_l, \boldsymbol{z}_j) = \frac{C}{C + ||\boldsymbol{z}_l - \boldsymbol{z}_j||_2^2}.
\end{align}
After training it is possible to sample from the chosen latent prior distribution, $p(\boldsymbol{z})$, pass it through the decoder, $\phi_{\text{dec}}$, and obtain a high-fidelity sample, $\phi_{\text{dec}}(\boldsymbol{z}) = \boldsymbol{q}$. 


\subsubsection{Supervised Wasserstein Autoencoders}
We here introduce an extra input to the decoder, $\boldsymbol{m}$, so that $\phi_{\text{enc}}(\boldsymbol{z}, \boldsymbol{m})$. This way the decoder models the conditional distribution, $P(\boldsymbol{q} | \boldsymbol{m})$. A visualization of the supervised WAE-MMD is shown in Figure \ref{fig:WAE-MMD}.

\subsubsection{Consistency Regularization}
As mentioned, the purpose of reducing the dimension of the state is to compute the dynamics in the low-dimensional latent space. Therefore, the evolution of the latent trajectory should be equivalent to solving the PDE directly. To achieve this, we make use of the findings in \cite{wan2023evolve}. Ideally, the latent dynamics model, the encoder, and the decoder should satisfy:
\begin{align} \label{eq:ideal_hf_time_derivative}
    \dot{\boldsymbol{q}} = \nabla_{\boldsymbol{z}} \phi_{\text{dec}}(\boldsymbol{z}) \dot{\boldsymbol{z}}, \quad 
    \dot{\boldsymbol{z}} = \nabla_{\boldsymbol{q}} \phi_{\text{enc}}(\boldsymbol{q}) \dot{\boldsymbol{q}}.
\end{align}
Due to the complexity of the PDEs and the autoencoder, this is, in general, not achievable. Instead, we can regularize the autoencoder without making use of the time derivatives directly. From \eqref{eq:ideal_hf_time_derivative}, we have:
\begin{align}
    \dot{\boldsymbol{q}} = \nabla_{\boldsymbol{z}} \phi_{\text{dec}}(\boldsymbol{z}) \nabla_{\boldsymbol{q}} \phi_{\text{enc}}(\boldsymbol{q}) \dot{\boldsymbol{q}}, \quad 
    \dot{\boldsymbol{z}} = \nabla_{\boldsymbol{q}} \phi_{\text{enc}}(\boldsymbol{q}) \nabla_{\boldsymbol{z}} \phi_{\text{dec}}(\boldsymbol{z}) \dot{\boldsymbol{z}},
\end{align}
which are the time-derivatives of
\begin{align}
    \boldsymbol{q} = \phi_{\text{dec}}(\phi_{\text{enc}}(\boldsymbol{q})), \quad 
    \boldsymbol{z} = \phi_{\text{enc}}(\phi_{\text{dec}}(\boldsymbol{z})).
\end{align}
The first equation naturally gives rise to the reconstruction loss, while the second equation gives rise to the consistency loss:
\begin{align}
    C(\phi_{\text{enc}}, \phi_{\text{dec}})  = ||\boldsymbol{z} - \phi_{\text{enc}}(\phi_{\text{dec}}(\boldsymbol{z}))||_2^2.
\end{align}
By adding the consistency loss to the WAE loss we thereby regularize the autoencoder to promote consistency:
\begin{align}
    L_{\text{WAE}}(\phi_{\text{enc}}, \phi_{\text{dec}}) 
    = 
    \frac{1}{N} \sum_{i=1}^{N} \left(\boldsymbol{q}_i - \phi_{\text{dec}}(\phi_{\text{enc}}(\boldsymbol{q}_i)) \right)^2
    +
    \lambda D(p(\boldsymbol{z}), p_{\text{enc}}(\boldsymbol{z}))
    + 
    \alpha R(\phi_{\text{enc}}, \phi_{\text{dec}})
    +
    \beta C(\phi_{\text{enc}}, \phi_{\text{dec}}),
\end{align}
where $\beta$ is an added hyperparameter. 

\subsection{Latent Space Time-stepping}
Once the AE is trained we can transform high-fidelity trajectories to latent space trajectories. However, we want to be able to compute the latent space trajectories in the latent space. That is, we want to be able to perform time stepping in the latent space. For this purpose, we make use of transformers. Transformers make use of so-called attention mechanisms and were first introduced in \cite{vaswani2017attention} as a NN model to deal natural language processing. It was later showed that transformers are highly useful for time series modeling as well. In \cite{geneva2022transformers} it is shown that transformers are highly suitable for modeling physical systems as they mimic the structure of multi-step methods. Therefore, we utilize them in this work. For an in-depth description of the transformer architecture, see Appendix \ref{appendix:attention_and_transformers} 

Time stepping in latent space is done by having a map, $f$, that advances a latent state in time:
\begin{align}
    \boldsymbol{z}_{n+1} = f(\boldsymbol{z}_n ; \boldsymbol{m}_n).
\end{align}
Adopting the mindset of multi step time integrators, we make use of several previous time steps to predict the next latent state:
\begin{align}
    \boldsymbol{z}_{n+1} = f(\boldsymbol{z}_{n-k:n} ; \boldsymbol{m}_n),
\end{align}
where $k$ is referred to as the memory. See Figure \ref{fig:transformer}. For multiple time steps we apply the transformer model recursively. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/transformer.pdf}
    \caption{Illustration of the transformer time stepping model.}
    \label{fig:transformer}
\end{figure}

After trajectories are computed in the latent space, high-fidelity trajectories are recovered by passing it through the decoder:
\begin{align}
    \left\{ \boldsymbol{z}_{0}, \boldsymbol{z}_{1}, \ldots, \boldsymbol{z}_{N_t}  \right\} \quad \rightarrow \quad \left\{ \phi_{\text{dec}}(\boldsymbol{z}_{0}), \phi_{\text{dec}}(\boldsymbol{z}_{1}), \ldots, \phi_{\text{dec}}(\boldsymbol{z}_{N_t})  \right\} = \left\{ \boldsymbol{q}_{0}, \boldsymbol{q}_{1}, \ldots, \boldsymbol{q}_{N_t}  \right\}.
\end{align}

\subsubsection{Parameterized Time-stepping}
In high-fidelity space the dynamics is not only dependent on the previous state, but also a set of parameters. This will also be the case for the latent dynamics. Hence, the latent space time-stepping model must include the parameters of interest as input. This can be done in several ways depending on the specific choice of neural network architectures. In this paper, we adopt the approach presented in \cite{han2022predicting}. Here, the parameters are encoded and added too the sequence of states as the first entry:
\begin{align}
    \left\{g(\boldsymbol{m}_n), \boldsymbol{z}_{n-k}, \boldsymbol{z}_{n-k+1}, \ldots, \boldsymbol{z}_{n}  \right\} \rightarrow f\left( \left\{g(\boldsymbol{m}_n), \boldsymbol{z}_{n-k}, \boldsymbol{z}_{n-k+1}, \ldots, \boldsymbol{z}_{n}  \right\}  \right) = \boldsymbol{z}_{n+1}
\end{align}
$g$ is a parameter encoder that lifts the vector of parameters to the same dimension as the latent state. This yields an efficient way of making use of the attention mechanism in the transformer architecture, as the attention between the parameters and the whole sequence of states are computed. See Figure \ref{fig:transformer} for a visualization of the parameterized time-stepping.



\subsection{Analysis of the Proposed Method}
For the analysis of the proposed method, we consider the slightly less general case where a whole batch of observations, $\boldsymbol{y}_{0:n}$ are available at once. We then aim to estimate the posterior density, $p(\boldsymbol{u}|\boldsymbol{y}_{0:n})$. Let $h(\boldsymbol{y}_{0:n} | \boldsymbol{u})$ be the likelihood, $f(\boldsymbol{u})$ the prior, and $\boldsymbol{u}\in \mathbb{R}^d$. In our case, $f$ is chosen as the proposal density. This setup does not compromise the generality of the derived results, but it does make the analysis easier \cite{quang2010insight}. 

The posterior is approximated by the empirical density:
\begin{align} \label{eq:discrete_posterior}
    p^N(\boldsymbol{u}) = \sum_{i=1}^N w_{n+1}^{i} \delta\left(\boldsymbol{u} - \boldsymbol{u}^{i}\right) \approx p(\boldsymbol{u}),
\end{align}
where
\begin{align}
    w^{i} = \frac{h(\boldsymbol{y}_{0:n} | \boldsymbol{u}^i)}{\sum_{j=1}^N h(\boldsymbol{y}_{0:n} | \boldsymbol{u}^j)}.
\end{align}
The empirical density is a discrete approximation of the true posterior made up of the $N$ particles.

From \cite{quang2010insight, le2004stability}, we know that the empirical posterior converges to the true posterior in the RMSE with the number of particles:
\begin{align}
\mathbb{E} \left[ \left(\langle \hat{p}^N, \varphi \rangle - \langle p^N, \varphi \rangle  \right)^2 \right]^{1/2} \leq  \frac{c_0}{\sqrt{N}} I(f, h) ||\varphi||,
\end{align}
where 
\begin{align}
I(f, h) = \frac{\sup_{\boldsymbol{u}} h(\boldsymbol{y}_{0:n} | \boldsymbol{u})}{ \int_{\mathbb{R}^d} h(\boldsymbol{y}_{0:n} | \boldsymbol{u}) f(\boldsymbol{u}) \text{d}\boldsymbol{u}}.
\end{align}
$\langle \cdot, \cdot \rangle$ is the inner product, $\varphi$ is a measurable test function and $||\varphi|| = \sup_x \varphi(x)$. The expectation is taken with respect to the particles distribution. The convergence rate is the same as for standard Monte Carlo methods, $N^{-1/2}$. While the convergence rate does not show explicit dependence on the state dimension, it has been shown that the particle filter performs poorly for large dimension \cite{quang2010insight}. Furthermore, properties of the transition density also affect the convergence. 

The integral, $I$, is the important term to analyze with respect to the dimension and the prior distribution, as the convergence in the number of particles is independent of both of these factors. 

\subsubsection{Convergence and Latent Dimension}







\subsubsection{The Importance of Probabilistic Structure in the Latent Space}
\begin{align}
h(\boldsymbol{y}_{0:n} | \boldsymbol{a}) &= p_{\boldsymbol{\eta}}( \boldsymbol{y}_{0:n} - H(\phi_{dec}(\boldsymbol{a})))
\end{align}



\subsubsection{Old attempt}























The posterior distribution for $\boldsymbol{a}_{0:n+1}$ is given by:
\begin{align}
    p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) \propto 
    \int 
    \underbrace{p(\boldsymbol{y}_{n+1}| \boldsymbol{a}_{n+1})}_{\text{likelihood}}
    \overbrace{p(\boldsymbol{a}_{n+1}| \boldsymbol{a}_{n})}^{\text{transition/prior probability}}
    \underbrace{p(\boldsymbol{a}_{n}| \boldsymbol{y}_{0:n})}_{\text{previous posterior}}
    \text{d}\boldsymbol{a}_{n}
\end{align}
The general idea of the particle filter is to approximate this integral with a weighted sum:
\begin{align}
    p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) \approx \sum_{i=1}^N w_{n+1}^{(i)} \delta\left(\boldsymbol{a}_{n+1} - \boldsymbol{a}_{n+1}^{(i)}\right).
\end{align}
There exists no general methodology for choosing the number of particles, $N$, such that the approximation is good. However, it is well-known that the dimension of state, $\boldsymbol{a}_{n}$, and the complexity of the integrand play a significant role in lowering the number of necessary particles. Therefore, we want to design our surrogate model such that the latent dimension is small and the integrand becomes simple. Lowering the dimensional is already given by using the standard autoencoder. However, reducing the complexity is not. This is why we make use of the WAE. 

Firstly, let's look at the individual terms in the integral and how they are affected by the complexity of the latent space:
\begin{itemize}
    \item The likelihood, $p(\boldsymbol{y}_{n+1}| \boldsymbol{a}_{0:n+1})$, is not affected but the latent distribution. 
    \item The old posterior, $p(\boldsymbol{a}_{n}| \boldsymbol{y}_{0:n})$, is affected indirectly from the previous time steps.
    \item The transition probability/prior, $p(\boldsymbol{a}_{n+1}| \boldsymbol{a}_{n})$, IS affected by the latent distribution!
\end{itemize}
If the latent time stepping model and the initial prior particles are perfect, then the following would be enough:
\begin{align}
    \boldsymbol{a}_{n+1} = f(\boldsymbol{a}_{n}).
\end{align}
However, we might not cover the entire density and the time-stepping model is not perfect. Hence, we need to model the error:
\begin{align}
    \boldsymbol{a}_{n+1} = f(\boldsymbol{a}_{n}) + \hat{\boldsymbol{\xi}}, \quad \hat{\boldsymbol{\xi}} \sim P(\hat{\boldsymbol{\xi}}).
\end{align}
It is a notoriously difficult problem to estimate the true model error distribution. 







\begin{comment}
    \begin{align*}
    p(\boldsymbol{q}_{n+1}| \boldsymbol{y}_{0:n+1}) &=
    \int p(\boldsymbol{q}_{n+1}|\boldsymbol{y}_{0:n+1}\boldsymbol{a}_{n+1}) p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) \text{d}\boldsymbol{a}_{n+1} \\
    &= \int p(\boldsymbol{q}_{n+1}|\boldsymbol{a}_{n+1}) p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) \text{d}\boldsymbol{a}_{n+1} \\
    &\propto \int p(\boldsymbol{q}_{n+1}|\boldsymbol{a}_{n+1}) p(\boldsymbol{y}_{n+1} | \boldsymbol{a}_{n+1}) p(\boldsymbol{a}_{n+1} | \boldsymbol{y}_{0:n})\text{d}\boldsymbol{a}_{n+1} \\
    &= \int p(\boldsymbol{q}_{n+1}|\boldsymbol{a}_{n+1}) p_{\zeta_n}(\boldsymbol{y}_{n+1} - h(\phi_{\text{dec}}(\boldsymbol{a}_{n+1})))p(\boldsymbol{a}_{n+1} | \boldsymbol{y}_{0:n})\text{d}\boldsymbol{a}_{n+1} 
\end{align*}


\begin{align*}
    \tilde{w}_{n+1}^{(i)} &= \tilde{w}(\boldsymbol{a}_{n+1}) \\
    &= w(\boldsymbol{a}_{n})p(\boldsymbol{y}_{n+1}|\boldsymbol{a}_{n+1}) \\
    &= w(\boldsymbol{a}_{n})p(\boldsymbol{y}_{n+1}|\boldsymbol{a}_{n+1})
\end{align*}


\begin{align*}
    p(\boldsymbol{q}_{n+1}| \boldsymbol{y}_{0:n+1}) &=
    \int p(\boldsymbol{q}_{n+1}|\boldsymbol{y}_{0:n+1}\boldsymbol{a}_{n+1}) p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) \text{d}\boldsymbol{a}_{n+1} \\
    &= \int p(\boldsymbol{q}_{n+1}|\boldsymbol{a}_{n+1}) p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) \text{d}\boldsymbol{a}_{n+1} \\
    &\propto \int p(\boldsymbol{q}_{n+1}|\boldsymbol{a}_{n+1}) p(\boldsymbol{y}_{n+1} | \boldsymbol{a}_{n+1}) p(\boldsymbol{a}_{n+1} | \boldsymbol{y}_{0:n})\text{d}\boldsymbol{a}_{n+1} \\
    &= \int p(\boldsymbol{q}_{n+1}|\boldsymbol{a}_{n+1}) p(\boldsymbol{y}_{n+1} | \boldsymbol{a}_{n+1}) \int p(\boldsymbol{a}_{n+1} | \boldsymbol{a}_{n}) p(\boldsymbol{a}_{n}| \boldsymbol{y}_{0:n}) \: \text{d}\boldsymbol{a}_n \text{d}\boldsymbol{a}_{n+1} 
\end{align*}

\begin{align*}
    p(\boldsymbol{a}_{n+1}| \boldsymbol{y}_{0:n+1}) &\propto  p(\boldsymbol{a}_{n+1} | \boldsymbol{y}_{0:n})  p(\boldsymbol{a}_{n+1} | \boldsymbol{y}_{0:n})\\
    &= p(\boldsymbol{y}_{n+1} | \boldsymbol{a}_{n+1}) \int p(\boldsymbol{a}_{n+1} | \boldsymbol{a}_{n}) p(\boldsymbol{a}_{n}| \boldsymbol{y}_{0:n}) \: \text{d}\boldsymbol{a}_n \\
    &\propto p(\boldsymbol{y}_{n+1} | \boldsymbol{a}_{n+1}) \int p(\boldsymbol{a}_{n+1} | \boldsymbol{a}_{n}) \int p(\boldsymbol{a}_{n} | \boldsymbol{a}_{n-1}) p(\boldsymbol{a}_{n-1}| \boldsymbol{y}_{0:n-1}) \: \text{d}\boldsymbol{a}_{n-1} \: \text{d}\boldsymbol{a}_n \\
    &= p(\boldsymbol{y}_{n+1} | \boldsymbol{a}_{n+1}) \int f_{\epsilon}(\boldsymbol{a}_{n}) \int f_{\epsilon}(\boldsymbol{a}_{n-1}) p(\boldsymbol{a}_{n-1}| \boldsymbol{y}_{0:n-1}) \: \text{d}\boldsymbol{a}_{n-1} \: \text{d}\boldsymbol{a}_n \\
\end{align*}

\begin{align}
    f_{\epsilon}(\boldsymbol{a}_{n}) = f(\boldsymbol{a}_{n}) + \epsilon
\end{align}

\subsection{New Try!}
\begin{align}
    p(\boldsymbol{a}_{0:n+1}| \boldsymbol{y}_{0:n+1}) &= \frac{p(\boldsymbol{a}_{0:n+1},\boldsymbol{y}_{0:n+1})}{p(\boldsymbol{y}_{0:n+1})} \\
    &= \frac{p(\boldsymbol{a}_{0:n+1})p(\boldsymbol{y}_{0:n+1}|\boldsymbol{a}_{0:n+1})}{p(\boldsymbol{y}_{0:n+1})}
\end{align}


\end{comment}




\section{Attention and Transformers} \label{appendix:attention_and_transformers}

We will give an overview and highlight the relevant features of the transformer architecture in this paper.  
The key to the transformer architecture is the so-called attention mechanism. The commonly used one is the scaled dot-product attention. For a matrix, $X\in\mathbb{R}^{k\times d}$, the scaled dot-product attention is computed by:
\begin{subequations} \label{eq:attention}
\begin{gather}
    K = F_k(X)\in\mathbb{R}^{k\times d}, \quad Q = F_q(X)\in\mathbb{R}^{k\times d}, \quad V= F_v(X)\in\mathbb{R}^{k\times d},  \\
    Attention(Q, K, V) =  softmax\left(\frac{QK^T}{\sqrt{d}}\right) V,
\end{gather}
\end{subequations}
$C$ is referred to as the attention map which is passed on for further computations. $K$ is referred to as the keys, $Q$ the queries, and $V$ the values. $F_k$, $F_q$, and $F_v$ are typically shallow neural networks to be fitted during training. $k$ is the context length and $d$ is the embedding dimension. An attention layer typically consists of multiple attention heads. Each head is of the same structure but consists of different functions $F_k$, $F_q$, and $F_v$. This results in multiple attention maps, $C_i$, that are concatenated along the $d$ dimension. 

By connecting the attention layer to  a residual connection, a normalization layer, a dense neural network, another residual connection and another normalization, we have the transformer encoder module. See Figure \ref{fig:transformer} for a visualization.

With $X$ a sequence of $k$ elements, with each element being a vector of size $d$, the attention mechanism computes how much each element in the sequence should attend to every other element. In the context of natural language processing, the attention mechanism computes how much every word in a sequence is influenced by any other word in the sequence. A slightly more suitable interpretation for our use case is to consider $X$ a graph with $k$ nodes and $d$ features in each node. The attention mechanism then computes how strong the connection should be between each pair of nodes.  

In Equation \eqref{eq:attention} the type of attention described is referred to as self-attention. This refers to the fact that all elements of $X$ only attend to other elements in $X$. Similarly, one defines cross-attention by using the attention map from another source as keys and values. By combining this with self-attention, normalization and a dense neural network, we have the decoder transformer module. 

The transformer encoder is not aware of the relative positions of the individual nodes. Therefore, a positional encoding is added to the features before passing them through the transformers.   



==> related_work.tex <==

\section*{Related Work}\label{paper_4:section:related_work}
The essential elements of the LSP filter are dimensionality reduction, surrogate modeling, and data assimilation, in particular in PDE-defined problems. 
 
\subsection*{Dimensionality Reduction}   
The autoencoder (AE) forms the common deep learning framework for data-driven dimensionality \cite{kingma2013auto, tolstikhin2017wasserstein}. An AE setup can be combined with different neural network architectures, with various convolutional and pooling layers \cite{mucke2021reduced, geneva2022transformers, wan2023evolve}. Convolutional layers  however tend to have inherent inductive biases and struggle with discontinuous signals, resulting in spurious oscillations. Transformers, originally developed for text processing, have proven effective for image processing in the form of vision transformers (ViT) \cite{dosovitskiy2020image}. These transformers divide images into patches and apply the attention mechanism between each set of patches. Yet, since there is no natural way of reducing or expanding the dimensionality of the data, the ViT has been used to dimensionality reduction tasks only to a limited degree \cite{ovadia2023vito,li2023ib,ran2022transformer, heo2021rethinking}. Importantly, current ViTs have not been integrated with increasing numbers of channels in convolutional layers to represent increasingly complicated features. 

\subsection*{Deep Learning-Based Surrogate Models} 
Numerous examples of deep learning-based surrogate models in scientific computing exist. In \cite{fresca2021comprehensive, wang2019non}, neural networks are trained non-intrusively to map parameters and to solve a PDE at specific times. While such approaches have shown great promise, they are not suitable for downstream tasks that are inherently time-sequential, such as online sequential data assimilation. For the latter, conventional architectures such as LSTMs and CNNs have  been developed to non-intrusively approximate parametric time stepping \cite{xu2020multi, mucke2021reduced}. Here, the neural network surrogate advances the state in time, conditioned on the provided parameters. 
Recent work has also explored alternative neural network architectures for surrogate models,  such as transformers, graph neural networks, and Fourier neural operators \cite{geneva2022transformers, ovadia2023vito, han2022predicting, li2020fourier}. 

\subsection*{Deep Learning for Data Assimilation}
In \cite{patel2020bayesian, xia2022bayesian, mucke2023markov}, generative deep learning is used for high-dimensional state- and parameter estimation. However, none of these approaches performs sequential assimilation of the data. In \cite{chen2023reduced, brunton2016discovering}, deep learning is used for model discovery. There, the model is a-priori unknown and is learned from the observations, requiring a large number of observations in space and time to recover the complete, unknown state; it is not yet clear how these methods perform with real-time data assimilation. In \cite{silva2023generative}, a GAN set-up, combined with proper orthogonal decomposition, is used for sequential data assimilation with an approach similar to randomized maximum likelihood. However, unlike particle filters, convergence of such methods is not ensured in nonlinear cases \cite{evensen2022data}. In \cite{yang2022particle}, a particle filter using a latent space formulation is presented. The approach evaluates the likelihood by iterative closest point registration fitness scores and the latent time stepping is only linear. It is unknown how the method would perform on highly nonlinear PDE-based problems with few observations in space and time. For a review of applications of deep learning for data assimilation, see \cite{cheng2023machine}.




